Safe, Fast, Concurrent Proof Checking for the lambda-Pi Calculus Modulo Rewriting

Several proof assistants, such as Isabelle or Coq, can concurrently check multiple proofs. In contrast, the vast majority of today's small proof checkers either does not support concurrency at all or only limited forms thereof, restricting the efficiency of proof checking on multi-core processors. This work shows the design of a small, memory- and thread-safe kernel that efficiently checks proofs both concurrently and non-concurrently. This design is implemented in a new proof checker called Kontroli for the lambda-Pi calculus modulo rewriting, which is an established framework to uniformly express a multitude of logical systems. Kontroli is faster than the reference proof checker for this calculus, Dedukti, on all of five evaluated datasets obtained from proof assistants and interactive theorem provers. Furthermore, Kontroli reduces the time of the most time-consuming part of proof checking using eight threads by up to 6.6x.

==> prftree/inference-rules.tex <==
\newcommand\typeinf{
\prftree[r]{}
{\phantom{A}}
{\Gamma, \Delta \vdash \Type : \Kind}
}
%
\newcommand\applinf{
\prftree[r]{}
{\Gamma, \Delta \vdash t : \Pi x\!:\!A.\, B}
{\Gamma, \Delta \vdash u : A}
{\Gamma, \Delta \vdash t\, u : B[u / x]}
}
%
\newcommand\abstinf{
\prftree[r]{}
{\Gamma, \Delta \left\{x \to A\right\} \vdash t : B}
{\Gamma, \Delta \vdash (\Pi x\!:\!A.\, B) : s}
{\Gamma, \Delta \vdash (\lambda x\!:\!A.\, t) : (\Pi x\!:\!A.\, B)}
}
%
\newcommand\prodinf{
\prftree[r]{}
{\Gamma, \Delta \vdash A : \Type}
{\Gamma, \Delta,\, x : A \vdash t : s}
{\Gamma, \Delta \vdash (\Pi x\!:\!A.\, t) : s}
}
%
\newcommand\convinf{
\prftree[r]{}
{\Gamma, \Delta \vdash t : A}
{\Gamma, \Delta \vdash B : s}
{A \sim _{\Gamma} B}
{\Gamma, \Delta \vdash t : B}
}
\centering
\begin{tabular}{m{\widthof{Typ}} m{\widthof{\abstinf}}}
Type & \mbox{\typeinf} \\[1.5em]
Appl & \mbox{\applinf} \\[1.5em]
Abst & \mbox{\abstinf} \\[1.5em]
Prod & \mbox{\prodinf} \\[1.5em]
Conv & \mbox{\convinf}
\end{tabular}
\par % needed for centering


==> tikz/execution.tex <==
\tikzset{
  block/.style = {draw, signal, signal from=west, signal to=east, text height=1.5ex, text depth=.25ex},
}

\centering

\subcaptionbox{Sequential processing.\label{fig:sequential}}
{\input{tikz/sequential}}

\vspace{\baselineskip}

\subcaptionbox{Parallel parsing.\label{fig:parallelc}}
{\input{tikz/parallelc}}

\vspace{\baselineskip}

\subcaptionbox{Parallel checking.\label{fig:parallelj}}
{\input{tikz/parallelj}}


==> tikz/itp-size.tex <==
% courtesy of: https://tex.stackexchange.com/a/116720
\pgfplotsset{
    mark repeat*/.style={
        scatter,
        scatter src=x,
        scatter/@pre marker code/.code={
            \pgfmathtruncatemacro\usemark{
                or(mod(\coordindex,#1)==0, (\coordindex==(\numcoords-1))
            }
            \ifnum\usemark=0
                \pgfplotsset{mark=none}
            \fi
        },
        scatter/@post marker code/.code={}
    }
}

% modified pgfplots `color` style by setting the mark of the third entry
% from `otimes*` to `triangle*` to increase the readability of the plot
\pgfplotscreateplotcyclelist{color'}{%
	blue,every mark/.append style={fill=blue!80!black},mark=*\\%
	red,every mark/.append style={fill=red!80!black},mark=square*\\%
	brown!60!black,every mark/.append style={fill=brown!80!black},mark=triangle*\\%
}

\begin{tikzpicture}
\begin{loglogaxis}
[ legend pos=north east
, xlabel=Commands
, y unit=B
, ylabel=Size
, mark repeat*={10000}
]
\pgfplotsset{cycle list name=color'}
\addplot table {eval/itp/size/isabelle_hol.dat};
\addlegendentry{Isabelle/HOL};
\addplot table {eval/itp/size/hol_stdlib_u.dat};
\addlegendentry{HOL Light};
\addplot table {eval/itp/size/matita_sttfa.dat};
\addlegendentry{Matita};
\end{loglogaxis}
\end{tikzpicture}


==> tikzlibrarypaths.ortho.code.tex <==
\let\tikz@orig@rect\tikz@rect
\def\tikz@rect{\pgfutil@ifnextchar e\tikz@orig@rect\qrr@tikz@r}
\def\qrr@tikz@r -{%
  \pgfutil@ifnextchar l\qrr@tikz@lr@lineto{%
    \pgfutil@ifnextchar r\qrr@tikz@rl@lineto{%
      \pgfutil@ifnextchar u\qrr@tikz@ud@lineto{%
        \pgfutil@ifnextchar d\qrr@tikz@du@lineto\tikz@expand
      }%
    }%
  }%
}
\let\tikz@orig@vh@lineto@next\tikz@vh@lineto@next
\def\tikz@vh@lineto@next{%
  \pgfutil@ifnextchar|{\expandafter\qrr@tikz@vhv@lineto\pgfutil@gobble}%
    {\pgfutil@ifnextchar\tikz@activebar{\expandafter\qrr@tikz@vhv@lineto\pgfutil@gobble}%
      {\tikz@orig@vh@lineto@next}}}
\let\tikz@orig@hv@lineto\tikz@hv@lineto
\def\tikz@hv@lineto{%
  \pgfutil@ifnextchar-{\expandafter\qrr@tikz@hvh@lineto\pgfutil@gobble}%
    {\tikz@orig@hv@lineto}}
\tikzset{%
  |-|/.style={%
   /utils/exec=\pgfmathsetmacro\qrr@tikz@hvvh@ratio{#1},%
   to path={|-| (\tikztotarget) \tikztonodes}},%
  -|-/.style={%
   /utils/exec=\pgfmathsetmacro\qrr@tikz@hvvh@ratio{#1},%
   to path={-|- (\tikztotarget) \tikztonodes}},%
  ud/.style={%
    udlr/ud distance/.expanded={#1},%
    to path={r-ud (\tikztotarget) \tikztonodes}},%
  du/.style={%
    udlr/du distance/.expanded={#1},%
    to path={r-du (\tikztotarget) \tikztonodes}},%
  lr/.style={%
    udlr/lr distance/.expanded={#1},%
    to path={r-lr (\tikztotarget) \tikztonodes}},%
  rl/.style={%
    udlr/rl distance/.expanded={#1},%
    to path={r-rl (\tikztotarget) \tikztonodes}},%
  ud/.default=\pgfkeysvalueof{/tikz/udlr/ud distance},%
  du/.default=\pgfkeysvalueof{/tikz/udlr/du distance},%
  rl/.default=\pgfkeysvalueof{/tikz/udlr/rl distance},%
  lr/.default=\pgfkeysvalueof{/tikz/udlr/lr distance},%
  |-|/.default=\qrr@tikz@hvvh@ratio,%
  -|-/.default=\qrr@tikz@hvvh@ratio
}

%BEGIN_FOLD hvvh operator
\def\qrr@tikz@vhv@lineto{\pgfutil@ifnextchar[{\qrr@tikz@collect@hvvh@options\qrr@tikz@vhv@lineto@next}{\qrr@tikz@collect@hvvh@options\qrr@tikz@vhv@lineto@next[]}}
\def\qrr@tikz@hvh@lineto{\pgfutil@ifnextchar[{\qrr@tikz@collect@hvvh@options\qrr@tikz@hvh@lineto@next}{\qrr@tikz@collect@hvvh@options\qrr@tikz@hvh@lineto@next[]}}
%END_FOLD

%BEGIN_FOLD udlr operators
%% ud style
\def\qrr@tikz@rl@lineto rl{\pgfutil@ifnextchar[{\qrr@tikz@collect@hvvh@options\qrr@tikz@rl@lineto@next}{\qrr@tikz@collect@hvvh@options\qrr@tikz@rl@lineto@next[]}}
\def\qrr@tikz@lr@lineto lr{\pgfutil@ifnextchar[{\qrr@tikz@collect@hvvh@options\qrr@tikz@lr@lineto@next}{\qrr@tikz@collect@hvvh@options\qrr@tikz@lr@lineto@next[]}}
\def\qrr@tikz@du@lineto du{\pgfutil@ifnextchar[{\qrr@tikz@collect@hvvh@options\qrr@tikz@du@lineto@next}{\qrr@tikz@collect@hvvh@options\qrr@tikz@du@lineto@next[]}}
\def\qrr@tikz@ud@lineto ud{\pgfutil@ifnextchar[{\qrr@tikz@collect@hvvh@options\qrr@tikz@ud@lineto@next}{\qrr@tikz@collect@hvvh@options\qrr@tikz@ud@lineto@next[]}}
%END_FOLD

\input tikzlibrarypaths.ortho.tex
\endinput


==> tikzlibrarypaths.ortho.tex <==
\newlength\qrr@tikz@udlr@distance
\newlength\qrr@tikz@hvvh@distance
\newif\ifqrr@tikz@hvvh@middle
\newif\ifqrr@tikz@hvvh@fromcenter
\newif\iftikz@ortho@preflush
\tikz@ortho@preflushtrue
\let\tikz@origtotarget\pgfutil@empty

%%% |-/-|
\tikzset{
  |-/.style={to path={|- (\tikztotarget) \tikztonodes}},
  -|/.style={to path={-| (\tikztotarget) \tikztonodes}},
  *|/.style={to path={%
    \pgfextra
      \iftikz@shapeborder
        \tikz@scan@one@point\pgfutil@firstofone(\tikztotarget)\relax
        \ifdim\pgf@y>\tikz@lasty\relax
          \edef\tikztostart{\tikztostart.north}%
        \else
          \edef\tikztostart{\tikztostart.south}%
        \fi
      \fi
    \endpgfextra
    (perpendicular cs: horizontal line through={(\tikztostart)},
                       vertical line through={(\tikztotarget)}) -- (\tikztotarget) \tikztonodes
  }},
  *-/.style={to path={%
    \pgfextra
      \iftikz@shapeborder
        \tikz@scan@one@point\pgfutil@firstofone(\tikztotarget)\relax
        \ifdim\pgf@x>\tikz@lastx\relax
          \edef\tikztostart{\tikztostart.east}%
        \else
          \edef\tikztostart{\tikztostart.west}%
        \fi
      \fi
    \endpgfextra
    (perpendicular cs: vertical line through={(\tikztostart)},
                     horizontal line through={(\tikztotarget)}) -- (\tikztotarget) \tikztonodes
  }},
  |*/.style={to path={%
    \pgfextra
      \tikz@scan@one@point\pgfutil@firstofone(\tikztotarget)\relax
      \iftikz@shapeborder
        \let\tikz@origtotarget\tikztotarget
        \ifdim\pgf@y>\tikz@lasty\relax
          \edef\tikztotarget{\tikztotarget.south}%
        \else
          \edef\tikztotarget{\tikztotarget.north}%
        \fi
      \fi
    \endpgfextra
    (\tikztostart) -- (perpendicular cs: vertical line through={(\tikztostart)},
                                         horizontal line through={(\tikztotarget)})
    \tikztonodes \ifx\tikz@origtotarget\pgfutil@empty\else\iftikz@ortho@preflush(\tikz@origtotarget)\fi\fi
  }},
  -*/.style={to path={%
    \pgfextra
      \tikz@scan@one@point\pgfutil@firstofone(\tikztotarget)\relax
      \iftikz@shapeborder
        \let\tikz@origtotarget\tikztotarget
        \ifdim\pgf@x>\tikz@lastx\relax
          \edef\tikztotarget{\tikztotarget.west}%
        \else
          \edef\tikztotarget{\tikztotarget.east}%
        \fi
      \fi
    \endpgfextra
    (\tikztostart) -- (perpendicular cs: horizontal line through={(\tikztostart)},
                                         vertical line through={(\tikztotarget)})
    \tikztonodes \ifx\tikz@origtotarget\pgfutil@empty\else\iftikz@ortho@preflush(\tikz@origtotarget)\fi\fi
  }},
  node as new start/.is if=tikz@ortho@preflush
}

%%% HVVH/UDLR
\tikzset{
  hvvh/.code={\pgfqkeys{/tikz/hvvh}{#1}},%
  udlr/.code={\pgfqkeys{/tikz/udlr}{#1}},%
%  hvvh/.search also=/tikz/udlr,%
  udlr/.search also=/tikz/hvvh,% endless loop?
  hvvh/middle 0 to 1/.style={hvvh/spacing=0},%
  hvvh/0 to 1/.style={hvvh/middle 0 to 1},%
  hvvh/from center/.is if=qrr@tikz@hvvh@fromcenter,%
  udlr/from center/.style={/tikz/hvvh/from center={#1}},
  udlr/from center/.default=true,
  hvvh/spacing/.code=%
    \ifcase#1\relax
      \qrr@tikz@hvvh@middletrue
      \def\qrr@tikz@hvvh@timing@parts{1}%
      \def\qrr@tikz@hvvh@timing@first{0}%
      \def\qrr@tikz@hvvh@timing@last{1}%
      \def\qrr@tikz@hvvh@timing@subtr{0}%
      \def\qrr@tikz@hvvh@timing@factor{1}%
    \else
      \qrr@tikz@hvvh@middlefalse
      \def\qrr@tikz@hvvh@timing@parts{#1}%
      \pgfmathreciprocal{#1}\let\qrr@tikz@hvvh@timing@first\pgfmathresult
      \pgfmathsetmacro\qrr@tikz@hvvh@timing@last{1-\pgfmathresult}%
      \pgfmathreciprocal{#1-2}%
      \let\qrr@tikz@hvvh@timing@subtr\pgfmathresult
      \pgfmathsetmacro\qrr@tikz@hvvh@timing@factor{1+2*\pgfmathresult}%
    \fi,
  hvvh/ratio/.code=\pgfmathsetmacro\qrr@tikz@hvvh@ratio{#1},
  hvvh/distance/.code=\pgfmathsetlength\qrr@tikz@hvvh@distance{#1}\let\qrr@tikz@hvvh@ratio\pgfutil@empty,%
  udlr/distance/.style={/tikz/udlr/ud distance={#1},/tikz/udlr/du distance={#1},/tikz/udlr/lr distance={#1},/tikz/udlr/rl distance={#1}},%
  udlr/ud distance/.initial=+.5cm,%
  udlr/du distance/.initial=+.5cm,%
  udlr/lr distance/.initial=+.5cm,%
  udlr/rl distance/.initial=+.5cm%
}
\tikzset{% default
  hvvh/ratio=.5,%
  hvvh/spacing=4%
}

%BEGIN_FOLD Timer
\def\tikz@timer@hvhline{%
  \pgf@process{\tikz@timer@start}\pgf@ya\pgf@y
  \pgf@process{\tikz@timer@end}\pgf@yc\pgf@y
  \pgf@process{\tikz@timer@middle}\pgf@xb\tikz@time pt%
  \ifdim\tikz@time pt<\qrr@tikz@hvvh@timing@first pt% first quarter
    \ifqrr@tikz@hvvh@middle
      \advance\pgf@xb1pt%
    \else
      \pgf@xb\qrr@tikz@hvvh@timing@parts\pgf@xb
    \fi
    \edef\tikz@marshal{\noexpand\pgftransformlineattime{\pgf@sys@tonumber{\pgf@xb}}{\noexpand\tikz@timer@start}{%
        \noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@ya}}}%
  \else
    \ifdim\tikz@time pt>\qrr@tikz@hvvh@timing@last pt% last quarter
      \ifqrr@tikz@hvvh@middle
        \advance\pgf@xb-1pt%
      \else
        \pgf@xb\qrr@tikz@hvvh@timing@parts\pgf@xb
      \fi
      \advance\pgf@xb\dimexpr-\qrr@tikz@hvvh@timing@parts pt+1pt\relax%
      \edef\tikz@marshal{\noexpand\pgftransformlineattime{\pgf@sys@tonumber{\pgf@xb}}%
        {\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@yc}}{\noexpand\tikz@timer@end}}%
    \else% middle half
      \pgf@xb\qrr@tikz@hvvh@timing@factor\pgf@xb%
      \advance\pgf@xb-\qrr@tikz@hvvh@timing@subtr pt%
      \edef\tikz@marshal{\noexpand\pgftransformlineattime{\pgf@sys@tonumber{\pgf@xb}}%
        {\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@ya}}{\noexpand\tikz@timer@middle}}%
    \fi\fi\tikz@marshal}
\def\tikz@timer@vhvline{%
  \pgf@process{\tikz@timer@start}\pgf@xa\pgf@x
  \pgf@process{\tikz@timer@end}\pgf@xc\pgf@x
  \pgf@process{\tikz@timer@middle}\pgf@xb\tikz@time pt%
  \ifdim\tikz@time pt<\qrr@tikz@hvvh@timing@first pt% first quarter
    \ifqrr@tikz@hvvh@middle
      \advance\pgf@xb1pt%
    \else
      \pgf@xb\qrr@tikz@hvvh@timing@parts\pgf@xb
    \fi
    \edef\tikz@marshal{\noexpand\pgftransformlineattime{\pgf@sys@tonumber{\pgf@xb}}{\noexpand\tikz@timer@start}{%
        \noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@y}}}%
  \else
    \ifdim\tikz@time pt>\qrr@tikz@hvvh@timing@last pt% last quarter
    \ifqrr@tikz@hvvh@middle
      \advance\pgf@xb-1pt%
    \else
      \pgf@xb\qrr@tikz@hvvh@timing@parts\pgf@xb
    \fi
      \advance\pgf@xb by\dimexpr-\qrr@tikz@hvvh@timing@parts pt+1pt\relax%
      \edef\tikz@marshal{\noexpand\pgftransformlineattime{\pgf@sys@tonumber{\pgf@xb}}%
        {\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@y}}{\noexpand\tikz@timer@end}}%
    \else% middle half
      \pgf@xb=\qrr@tikz@hvvh@timing@factor\pgf@xb
      \advance\pgf@xb by-\qrr@tikz@hvvh@timing@subtr pt%
      \edef\tikz@marshal{\noexpand\pgftransformlineattime{\pgf@sys@tonumber{\pgf@xb}}%
        {\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@y}}{\noexpand\tikz@timer@middle}}%
      \fi\fi\tikz@marshal}

%END_FOLD
\let\tikz@hvvh@currentoption\pgfutil@empty
\def\qrr@tikz@collect@hvvh@options#1[#2]{\edef\tikz@hvvh@currentoption{#2}#1}
\def\qrr@tikz@hvh@lineto@next{%
  \pgfutil@ifnextchar n{\tikz@collect@label@onpath\qrr@tikz@hvh@lineto@next}
    {\pgfutil@ifnextchar c{\tikz@collect@coordinate@onpath\qrr@tikz@hvh@lineto@next}%
      {\pgfutil@ifnextchar p{\tikz@collect@pic@onpath\qrr@tikz@hvh@lineto@next}{\tikz@scan@one@point\qrr@tikz@@hvh@lineto}}}}
\def\qrr@tikz@vhv@lineto@next{%
  \pgfutil@ifnextchar n{\tikz@collect@label@onpath\qrr@tikz@vhv@lineto@next}
    {\pgfutil@ifnextchar c{\tikz@collect@coordinate@onpath\qrr@tikz@vhv@lineto@next}%
      {\pgfutil@ifnextchar p{\tikz@collect@pic@onpath\qrr@tikz@vhv@lineto@next}{\tikz@scan@one@point\qrr@tikz@@vhv@lineto}}}}
\def\qrr@tikz@ud@lineto@next{%
  \pgfutil@ifnextchar n{\tikz@collect@label@onpath\qrr@tikz@ud@lineto@next}
    {\pgfutil@ifnextchar c{\tikz@collect@coordinate@onpath\qrr@tikz@ud@lineto@next}
      {\pgfutil@ifnextchar p{\tikz@collect@pic@onpath\qrr@tikz@ud@lineto@next}{\tikz@scan@one@point\qrr@tikz@@ud@lineto}}}}
\def\qrr@tikz@du@lineto@next{%
  \pgfutil@ifnextchar n{\tikz@collect@label@onpath\qrr@tikz@du@lineto@next}
    {\pgfutil@ifnextchar c{\tikz@collect@coordinate@onpath\qrr@tikz@du@lineto@next}
      {\pgfutil@ifnextchar p{\tikz@collect@pic@onpath\qrr@tikz@du@lineto@next}{\tikz@scan@one@point\qrr@tikz@@du@lineto}}}}
\def\qrr@tikz@lr@lineto@next{%
  \pgfutil@ifnextchar n{\tikz@collect@label@onpath\qrr@tikz@lr@lineto@next}
    {\pgfutil@ifnextchar c{\tikz@collect@coordinate@onpath\qrr@tikz@lr@lineto@next}
      {\pgfutil@ifnextchar p{\tikz@collect@pic@onpath\qrr@tikz@lr@lineto@next}{\tikz@scan@one@point\qrr@tikz@@lr@lineto}}}}
\def\qrr@tikz@rl@lineto@next{%
  \pgfutil@ifnextchar n{\tikz@collect@label@onpath\qrr@tikz@rl@lineto@next}
    {\pgfutil@ifnextchar c{\tikz@collect@coordinate@onpath\qrr@tikz@rl@lineto@next}
      {\pgfutil@ifnextchar p{\tikz@collect@pic@onpath\qrr@tikz@rl@lineto@next}{\tikz@scan@one@point\qrr@tikz@@rl@lineto}}}}

\def\tikz@do@hvvh#1#2#3#4#5{%
% #1 = first kink
% #2 = second kink
% #3 = end
% #4 = timer
% #5 = tikz@shapeborder@name
  \pgfpathlineto{#1}%
  \pgfpathlineto{#2}%
  \pgfpathlineto{#3}%
  \def\tikz@timer@middle{#2}%
  \def\tikz@timer@end{#3}%
  \let\tikz@timer#4
  \edef\pgf@temp{#5}%
  \ifx\pgf@temp\pgfutil@empty
    \let\tikz@moveto@waiting\relax
  \else
    \edef\tikz@moveto@waiting{#5}%
  \fi
  \tikz@scan@next@command%
}
%BEGIN_FOLD hvvh operator
%% -|- operator
\def\qrr@tikz@@hvh@lineto#1{%
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \pgf@xb=\tikz@lastx
  \pgf@xc=\tikz@lastx
  \pgf@yc=\tikz@lasty
  \tikz@make@last@position{#1}%
  \tikz@flush@moveto@toward{\pgfqpoint{\tikz@lastx}{\pgf@yc}}\pgf@xc\pgf@yc
  \begingroup
    \pgfqkeys{/tikz/hvvh}{/tikz/style/.expand once=\tikz@hvvh@currentoption}%
    \iftikz@shapeborder
      \pgf@process{\pgfpointshapeborder{\tikz@shapeborder@name}{\pgfqpoint{\pgf@xb}{\tikz@lasty}}}%
      \ifqrr@tikz@hvvh@fromcenter
        \pgf@xc\pgf@xb
      \fi
      \ifx\qrr@tikz@hvvh@ratio\pgfutil@empty
        \ifdim\qrr@tikz@hvvh@distance<0pt\relax
          \ifqrr@tikz@hvvh@fromcenter
            \pgf@xc\tikz@lastx
          \else
            \pgf@xc\pgf@x
          \fi
        \fi
        \ifdim\pgf@x>\tikz@lastx
          \qrr@tikz@hvvh@distance-\qrr@tikz@hvvh@distance
        \fi
      \else
        \ifqrr@tikz@hvvh@fromcenter
          \qrr@tikz@hvvh@distance\tikz@lastx
        \else
          \qrr@tikz@hvvh@distance\pgf@x
        \fi
        \advance\qrr@tikz@hvvh@distance-\pgf@xc
        \qrr@tikz@hvvh@distance\qrr@tikz@hvvh@ratio\qrr@tikz@hvvh@distance
      \fi
      \advance\pgf@xc\qrr@tikz@hvvh@distance
      \edef\pgf@tempa{\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
      \edef\pgf@tempb{\noexpand\pgfqpoint{\the\pgf@xc}{\the\tikz@lasty}}%
      \edef\pgf@temp{\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
    \else
      \let\tikz@shapeborder@name\pgfutil@empty
      \ifqrr@tikz@hvvh@fromcenter
        \pgf@xc\pgf@xb
      \fi
      \ifx\qrr@tikz@hvvh@ratio\pgfutil@empty
        \ifdim\qrr@tikz@hvvh@distance<0pt\relax
          \pgf@xc\tikz@lastx
        \fi
        \ifdim\pgf@x>\tikz@lastx
          \qrr@tikz@hvvh@distance-\qrr@tikz@hvvh@distance
        \fi
      \else
        \qrr@tikz@hvvh@distance\tikz@lastx
        \advance\qrr@tikz@hvvh@distance-\pgf@xc
        \qrr@tikz@hvvh@distance\qrr@tikz@hvvh@ratio\qrr@tikz@hvvh@distance
      \fi
      \advance\pgf@xc\qrr@tikz@hvvh@distance
      \edef\pgf@tempa{\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
      \edef\pgf@tempb{\noexpand\pgfqpoint{\the\pgf@xc}{\the\tikz@lasty}}%
      \edef\pgf@temp{\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
    \fi%
    \xdef\pgf@marshal{%
      \noexpand\tikz@do@hvvh
        {\expandafter\noexpand\pgf@tempa}%
        {\expandafter\noexpand\pgf@tempb}%
        {\expandafter\noexpand\pgf@temp}%
        {\noexpand\tikz@timer@hvhline}{\tikz@shapeborder@name}}%
  \endgroup
  \pgf@marshal}

%% |-| operator
\def\qrr@tikz@@vhv@lineto#1{%
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \pgf@xc=\tikz@lastx
  \pgf@yb=\tikz@lasty
  \pgf@yc=\tikz@lasty
  \tikz@make@last@position{#1}%
  \tikz@flush@moveto@toward{\pgfqpoint{\pgf@xc}{\tikz@lasty}}\pgf@xc\pgf@yc
  \begingroup
    \pgfqkeys{/tikz/hvvh}{/tikz/style/.expand once=\tikz@hvvh@currentoption}%
    \iftikz@shapeborder
      \pgf@process{\pgfpointshapeborder{\tikz@shapeborder@name}{\pgfqpoint{\tikz@lastx}{\pgf@yb}}}%
      \ifqrr@tikz@hvvh@fromcenter
        \pgf@yc\pgf@yb
      \fi
      \ifx\qrr@tikz@hvvh@ratio\pgfutil@empty
        \ifdim\qrr@tikz@hvvh@distance<0pt\relax
          \ifqrr@tikz@hvvh@fromcenter
            \pgf@yc\tikz@lasty
          \else
            \pgf@yc\pgf@y
          \fi
        \fi
        \ifdim\pgf@y>\tikz@lasty
          \qrr@tikz@hvvh@distance-\qrr@tikz@hvvh@distance
        \fi
      \else
        \ifqrr@tikz@hvvh@fromcenter
          \qrr@tikz@hvvh@distance\tikz@lasty
        \else
          \qrr@tikz@hvvh@distance\pgf@y
        \fi
        \advance\qrr@tikz@hvvh@distance-\pgf@yc
        \qrr@tikz@hvvh@distance\qrr@tikz@hvvh@ratio\qrr@tikz@hvvh@distance
      \fi
      \advance\pgf@yc\qrr@tikz@hvvh@distance
      \edef\pgf@tempa{\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
      \edef\pgf@tempb{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\pgf@yc}}%
      \edef\pgf@temp{\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
    \else
      \let\tikz@shapeborder@name\pgfutil@empty
      \ifqrr@tikz@hvvh@fromcenter
        \pgf@yc\pgf@yb
      \fi
      \ifx\qrr@tikz@hvvh@ratio\pgfutil@empty
        \ifdim\qrr@tikz@hvvh@distance<0pt\relax
          \pgf@yc\tikz@lasty
        \fi
        \ifdim\pgf@y>\tikz@lasty
          \qrr@tikz@hvvh@distance-\qrr@tikz@hvvh@distance
        \fi
      \else
        \qrr@tikz@hvvh@distance\tikz@lasty
        \advance\qrr@tikz@hvvh@distance-\pgf@yc
        \qrr@tikz@hvvh@distance\qrr@tikz@hvvh@ratio\qrr@tikz@hvvh@distance
      \fi
      \advance\pgf@yc\qrr@tikz@hvvh@distance
      \edef\pgf@tempa{\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
      \edef\pgf@tempb{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\pgf@yc}}%
      \edef\pgf@temp{\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
    \fi%
    \xdef\pgf@marshal{%
      \noexpand\tikz@do@hvvh
        {\expandafter\noexpand\pgf@tempa}%
        {\expandafter\noexpand\pgf@tempb}%
        {\expandafter\noexpand\pgf@temp}%
        {\noexpand\tikz@timer@vhvline}{\tikz@shapeborder@name}}%
  \endgroup
  \pgf@marshal}

%% ud operator
\def\qrr@tikz@@ud@lineto#1{%
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \pgf@xc\tikz@lastx
  \pgf@yb\tikz@lasty
  \advance\tikz@lasty1pt%
  \let\pgf@temp\tikz@moveto@waiting
  \tikz@flush@moveto@toward{\pgfqpoint{\tikz@lastx}{\tikz@lasty}}\pgf@xc\pgf@yc
  \tikz@make@last@position{#1}%
  \begingroup
    \pgfqkeys{/tikz/udlr}{/tikz/style/.expand once=\tikz@hvvh@currentoption}%
    \pgfmathsetlength\qrr@tikz@udlr@distance{\pgfkeysvalueof{/tikz/udlr/ud distance}}%
    \iftikz@shapeborder
      \advance\pgf@y1pt%
      \pgf@process{\pgfpointshapeborder{\tikz@shapeborder@name}{\pgfqpoint{\pgf@x}{\pgf@y}}}%
      \ifqrr@tikz@hvvh@fromcenter
        \pgf@yc\pgf@yb
      \else\ifx\pgf@temp\relax
          \pgf@yc\pgf@yb
        \fi
      \fi
      \ifdim\pgf@yc<\pgf@y
        \ifqrr@tikz@hvvh@fromcenter
          \pgf@yc=\tikz@lasty
        \else
          \pgf@yc=\pgf@y
        \fi
      \fi
      \advance\pgf@yc\qrr@tikz@udlr@distance
      \edef\pgf@temp{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
    \else
      \let\tikz@shapeborder@name\pgfutil@empty
      \ifx\pgf@temp\relax\else
        \ifqrr@tikz@hvvh@fromcenter\else
          \pgf@yb\pgf@yc
        \fi
      \fi
      \ifdim\pgf@yb<\tikz@lasty\pgf@yb\tikz@lasty\fi
      \advance\pgf@yb\qrr@tikz@udlr@distance
      \pgf@yc\pgf@yb
      \edef\pgf@temp{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
    \fi
    \xdef\pgf@marshal{%
      \noexpand\tikz@do@hvvh
        {\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
        {\noexpand\pgfqpoint{\the\tikz@lastx}{\the\pgf@yc}}%
        {\expandafter\noexpand\pgf@temp}%
        {\noexpand\tikz@timer@vhvline}{\tikz@shapeborder@name}}%
  \endgroup
  \pgf@marshal}

%% du operator
\def\qrr@tikz@@du@lineto#1{%
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \pgf@xc\tikz@lastx
  \pgf@yb\tikz@lasty
  \advance\tikz@lasty-1pt%
  \let\pgf@temp\tikz@moveto@waiting
  \tikz@flush@moveto@toward{\pgfqpoint{\tikz@lastx}{\tikz@lasty}}\pgf@xc\pgf@yc
  \tikz@make@last@position{#1}%
  \begingroup
    \pgfqkeys{/tikz/udlr}{/tikz/style/.expand once=\tikz@hvvh@currentoption}%
    \pgfmathsetlength\qrr@tikz@udlr@distance{\pgfkeysvalueof{/tikz/udlr/du distance}}%
    \iftikz@shapeborder
      \advance\pgf@y-1pt%
      \pgf@process{\pgfpointshapeborder{\tikz@shapeborder@name}{\pgfqpoint{\pgf@x}{\pgf@y}}}%
      \ifqrr@tikz@hvvh@fromcenter
        \pgf@yc\pgf@yb
      \else\ifx\pgf@temp\relax
          \pgf@yc\pgf@yb
        \fi
      \fi
      \ifdim\pgf@yc>\pgf@y
        \ifqrr@tikz@hvvh@fromcenter
          \pgf@yc=\tikz@lasty
        \else
          \pgf@yc=\pgf@y
        \fi
      \fi
      \advance\pgf@yc-\qrr@tikz@udlr@distance
      \edef\pgf@temp{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
    \else
      \let\tikz@shapeborder@name\pgfutil@empty
      \ifx\pgf@temp\relax\else
        \ifqrr@tikz@hvvh@fromcenter\else
          \pgf@yb\pgf@yc
        \fi
      \fi
      \ifdim\pgf@yb>\tikz@lasty\pgf@yb\tikz@lasty\fi
      \advance\pgf@yb-\qrr@tikz@udlr@distance
      \pgf@yc\pgf@yb
      \edef\pgf@temp{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
    \fi
    \xdef\pgf@marshal{%
      \noexpand\tikz@do@hvvh
        {\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
        {\noexpand\pgfqpoint{\the\tikz@lastx}{\the\pgf@yc}}%
        {\expandafter\noexpand\pgf@temp}%
        {\noexpand\tikz@timer@vhvline}{\tikz@shapeborder@name}}%
  \endgroup
  \pgf@marshal}

%% lr operator
\def\qrr@tikz@@lr@lineto#1{%
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \pgf@xb\tikz@lastx
  \pgf@yc\tikz@lasty
  \advance\tikz@lastx-1pt%
  \let\pgf@temp\tikz@moveto@waiting
  \tikz@flush@moveto@toward{\pgfqpoint{\tikz@lastx}{\tikz@lasty}}\pgf@xc\pgf@yc
  \tikz@make@last@position{#1}%
  \begingroup
    \pgfqkeys{/tikz/udlr}{/tikz/style/.expand once=\tikz@hvvh@currentoption}%
    \pgfmathsetlength\qrr@tikz@udlr@distance{\pgfkeysvalueof{/tikz/udlr/lr distance}}%
    \iftikz@shapeborder
      \advance\pgf@x-1pt%
      \pgf@process{\pgfpointshapeborder{\tikz@shapeborder@name}{\pgfqpoint{\pgf@x}{\pgf@y}}}%
      \ifqrr@tikz@hvvh@fromcenter
        \pgf@xc\pgf@xb
      \else\ifx\pgf@temp\relax
          \pgf@xc\pgf@xb
        \fi
      \fi
      \ifdim\pgf@xc>\pgf@x
        \ifqrr@tikz@hvvh@fromcenter
          \pgf@xc=\tikz@lastx
        \else
          \pgf@xc=\pgf@x
        \fi
      \fi
      \advance\pgf@xc-\qrr@tikz@udlr@distance
      \edef\pgf@temp{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
    \else
      \let\tikz@shapeborder@name\pgfutil@empty
      \ifx\pgf@temp\relax\else
        \ifqrr@tikz@hvvh@fromcenter\else
          \pgf@xb\pgf@xc
        \fi
      \fi
      \ifdim\pgf@xb>\tikz@lastx\pgf@xb\tikz@lastx\fi
      \advance\pgf@xb-\qrr@tikz@udlr@distance
      \pgf@xc\pgf@xb
      \edef\pgf@temp{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
    \fi
    \xdef\pgf@marshal{%
      \noexpand\tikz@do@hvvh
        {\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
        {\noexpand\pgfqpoint{\the\pgf@xc}{\the\tikz@lasty}}%
        {\expandafter\noexpand\pgf@temp}%
        {\noexpand\tikz@timer@hvhline}{\tikz@shapeborder@name}}%
  \endgroup
  \pgf@marshal}

%% rl operator
\def\qrr@tikz@@rl@lineto#1{%
  \edef\tikz@timer@start{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
  \pgf@xb\tikz@lastx
  \pgf@yc\tikz@lasty
  \advance\tikz@lastx1pt%
  \let\pgf@temp\tikz@moveto@waiting
  \tikz@flush@moveto@toward{\pgfqpoint{\tikz@lastx}{\tikz@lasty}}\pgf@xc\pgf@yc
  \tikz@make@last@position{#1}%
  \begingroup
    \pgfqkeys{/tikz/udlr}{/tikz/style/.expand once=\tikz@hvvh@currentoption}%
    \pgfmathsetlength\qrr@tikz@udlr@distance{\pgfkeysvalueof{/tikz/udlr/rl distance}}%
    \iftikz@shapeborder%
      \advance\pgf@x1pt%
      \pgf@process{\pgfpointshapeborder{\tikz@shapeborder@name}{\pgfqpoint{\pgf@x}{\pgf@y}}}%
      \ifqrr@tikz@hvvh@fromcenter
        \pgf@xc\pgf@xb
      \else\ifx\pgf@temp\relax
          \pgf@xc\pgf@xb
        \fi
      \fi
      \ifdim\pgf@xc<\pgf@x
        \ifqrr@tikz@hvvh@fromcenter
          \pgf@xc=\tikz@lastx
        \else
          \pgf@xc=\pgf@x
        \fi
      \fi
      \advance\pgf@xc\qrr@tikz@udlr@distance
      \edef\pgf@temp{\noexpand\pgfqpoint{\the\pgf@x}{\the\pgf@y}}%
    \else
      \let\tikz@shapeborder@name\pgfutil@empty%
      \ifx\pgf@temp\relax\else
        \ifqrr@tikz@hvvh@fromcenter\else
          \pgf@xb\pgf@xc
        \fi
      \fi
      \ifdim\pgf@xb<\tikz@lastx\pgf@xb\tikz@lastx\fi
      \advance\pgf@xb\qrr@tikz@udlr@distance
      \pgf@xc\pgf@xb
      \edef\pgf@temp{\noexpand\pgfqpoint{\the\tikz@lastx}{\the\tikz@lasty}}%
    \fi
    \xdef\pgf@marshal{%
      \noexpand\tikz@do@hvvh
        {\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
        {\noexpand\pgfqpoint{\the\pgf@xc}{\the\tikz@lasty}}%
        {\expandafter\noexpand\pgf@temp}%
        {\noexpand\tikz@timer@hvhline}{\tikz@shapeborder@name}}%
  \endgroup
  \pgf@marshal}
%END_FOLD
\endinput

